Aggregating Votes with Local Differential Privacy: Usefulness, Soundness vs. Indistinguishability

Voting plays a central role in bringing crowd wisdom to collective decision making, meanwhile data privacy has been a common ethical/legal issue in eliciting preferences from individuals. This work studies the problem of aggregating individual's voting data under the local differential privacy setting, where usefulness and soundness of the aggregated scores are of major concern. One naive approach to the problem is adding Laplace random noises, however, it makes aggregated scores extremely fragile to new types of strategic behaviors tailored to the local privacy setting: data amplification attack and view disguise attack. The data amplification attack means an attacker's manipulation power is amplified by the privacy-preserving procedure when contributing a fraud vote. The view disguise attack happens when an attacker could disguise malicious data as valid private views to manipulate the voting result. In this work, after theoretically quantifying the estimation error bound and the manipulating risk bound of the Laplace mechanism, we propose two mechanisms improving the usefulness and soundness simultaneously: the weighted sampling mechanism and the additive mechanism. The former one interprets the score vector as probabilistic data. Compared to the Laplace mechanism for Borda voting rule with $d$ candidates, it reduces the mean squared error bound by half and lowers the maximum magnitude risk bound from $+\infty$ to $O(\frac{d^3}{n\epsilon})$. The latter one randomly outputs a subset of candidates according to their total scores. Its mean squared error bound is optimized from $O(\frac{d^5}{n\epsilon^2})$ to $O(\frac{d^4}{n\epsilon^2})$, and its maximum magnitude risk bound is reduced to $O(\frac{d^2}{n\epsilon})$. Experimental results validate that our proposed approaches averagely reduce estimation error by $50\%$ and are more robust to adversarial attacks.

==> abandon.tex <==
Enforcing local privacy degrades the usefulness of candidates' scores, while the Laplace approach also makes final scores extremely fragile to new types of strategic behaviors: privacy-amplified attack and privacy-concealed attack. By privacy-amplified attack, an attacker's constructive/deconstructive power is probabilistically amplified due to privacy preserving protocal. By privacy-concealed attach, an attacker could adversarially disguise  private views of voting profiles for manipulating the voting resluts. 

After theoretically analyzing the score estimaion error bounds in the non-strategic scenario and the manupulating risk bounds in the strategic scenario for the Laplace mechanism, we propose two novel approaches improving usefulness and robustness simultaneously: the weighted sampling mechansim and the additive mechanism. The weighted sampling mechanism interpretes the intercepted score vector as probabilistic data, improving the mean squared estimation error from $a$ to $b$, and the mean absolute risk from $c$ to $d$. The addtive mechanism 

, and ensures distinguishability on outputs no matter the true vote an voter holds

and define the domain with filtering parameter $p$ as follows:
$$\tilde{\mathcal{D}}_p=\{\tilde{v}\ |\ \tilde{v}\in \mathcal{R}^m,\ \text{Pr}[\tilde{v}|v] \geq p\ \text{for\ some}\  v\in \mathcal{D}\},$$
the filtered domain $\tilde{\mathcal{D}}_p$ of Laplace approach is:
$$\{\tilde{v}\ |\ \tilde{v}\in \mathcal{R}^m,\ |\tilde{v}-v|\leq \frac{\Delta(\log(1/p)+m\log(\Delta/\epsilon))}{\epsilon}\ \text{for\ some}\  v\in \mathcal{D}\},$$


\subsubsection{Usefulness metrics}
The estimators of average scores $\tilde{\theta}$ given by different mechanism uaually have varied accuracy, one accuracy measure we use is the mean squared error (MSE):
$$\text{error}_{\text{MSE}}=\mathbb{E}[|\tilde{\theta}-\theta|_2^2],$$
%another accuracy measure is the total variation error (TVE):
%$$\text{TVE}=\mathbb{E}[|\tilde{\theta}-\theta|_1].$$
%Since average scores eventually determines one winning candidates, we also use maximum absolute error (MAE) as a accuracy metric:
another accuracy measure is the maximum absolute error (MAE):
$$\text{error}_{\text{MAE}}=\mathbb{E}[\max_{j\in [1, d]}|\tilde{\theta}_j-\theta_j|].$$    


Since average scores are eventually used to determine one winning candidates, let $j_{max} = \arg \max_{j\in [1, d]} \theta_{j}$ denote the candidate's index with maximum average score in true average scores $\theta$, and $\tilde{j}_{max}=\arg \max_{j\in [1, d]} \tilde{\theta}_j$ denote the winning candidate's index in the estimated avearage scores $\tilde{\theta}$, one straight-forward measure is accuracy of winner (AOW):
$$\text{accuracy}_{\text{AOW}}=\mathbb{E}[\tilde{j}_{max} == j_{max}],$$
another measure is expected loss of winner (LOW):
$$\text{error}_{\text{LOW}}=\mathbb{E}[\theta_{j_{max}}-\theta_{\tilde{j}_{max}}],$$
